FSCNMF: Fusing Structure and Content via Non-negative Matrix Factorization for Embedding Information Networks

Analysis and visualization of an information network can be facilitated better using an appropriate embedding of the network. Network embedding learns a compact low-dimensional vector representation for each node of the network, and uses this lower dimensional representation for different network analysis tasks. Only the structure of the network is considered by a majority of the current embedding algorithms. However, some content is associated with each node, in most of the practical applications, which can help to understand the underlying semantics of the network. It is not straightforward to integrate the content of each node in the current state-of-the-art network embedding methods. In this paper, we propose a nonnegative matrix factorization based optimization framework, namely FSCNMF which considers both the network structure and the content of the nodes while learning a lower dimensional representation of each node in the network. Our approach systematically regularizes structure based on content and vice versa to exploit the consistency between the structure and content to the best possible extent. We further extend the basic FSCNMF to an advanced method, namely FSCNMF++ to capture the higher order proximities in the network. We conduct experiments on real world information networks for different types of machine learning applications such as node clustering, visualization, and multi-class classification. The results show that our method can represent the network significantly better than the state-of-the-art algorithms and improve the performance across all the applications that we consider.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

==> derivations1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plain Cover Letter
% LaTeX Template
% Version 1.0 (28/5/13)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% Original author:
% Rensselaer Polytechnic Institute
% http://www.rpi.edu/dept/arc/training/latex/resumes/
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------

% %\documentclass[11pt]{article} % Default font size of the document, change to 10pt to fit more text
% \usepackage{amsthm}
% \usepackage{newcent} % Default font is the New Century Schoolbook PostScript font
% \usepackage{helvet} % Uncomment this (while commenting the above line) to use the Helvetica font
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% % Margins
% %\topmargin=-1in % Moves the top of the document 1 inch above the default
% %\textheight=9.0in % Total height of the text on the page before text goes on to the next page, this can be increased in a longer letter
% %\oddsidemargin=-10pt % Position of the left margin, can be negative or positive if you want more or less room
% %\textwidth=6.75in % Total width of the text, increase this if the left margin was decreased and vice-versa

% %\let\raggedleft\raggedright % Pushes the date (at the top) to the left, comment this line to have the date on the right
% \include{macros}
% %\usepackage{amsmath}
% \begin{document}
% %----------------------------------------------------------------------------------------
% %	ADDRESSEE SECTION
% %----------------------------------------------------------------------------------------
% \vspace{-8pt}
% %\begin{letter}{Additions
% %}
% %\date{22nd January 2018}
% \begin{center}
% \large\bf Derivations
% \end{center}
% \vfill
% %\signature{Sambaran and Aswin} % Your name for the signature at the bottom
% %----------------------------------------------------------------------------------------
% %	LETTER CONTENT SECTION
% %----------------------------------------------------------------------------------------
%\opening{To be Added:}
The basic problem can be stated as follows.
\begin{align*}
& \min_{U,V} \hspace{4mm} D_2(U,V) = \frac{1}{2} \|C-UV \|_{F}^2 + \frac{\beta_1}{2} \|U-B \|_{F}^2 + \frac{\beta_2}{2} \|U\|_{F}^2 + \frac{\beta_3}{2} \| V \|_{F}^2 \\
\\ \vspace{1mm} \\
& \text{Update Rules:} \\
& U_{k+1} = U_k \times P_k^U \\
& V_{k+1} = V_k \times P_k^V.
\end{align*}
In the space of ``U'', this can be further written as follows.
\begin{align*}
& \min_{p_k^U} \hspace{4mm}  f(U_kP_k^U, C) = \frac{1}{2} \|C-U_kV_kP_k^U \|_{F}^2 + \frac{\beta_1}{2} \|U_kP_k^U-B \|_{F}^2 + \frac{\beta_2}{2} \|U_kP_k^U\|_{F}^2.
\end{align*}
In a scalar space, this leads to the below stated first order conditions.
$$(C-U_kV_kP_k^U) (-U_kV_k) + \beta_1 (U_kP_k^U-B)U_k + \beta_2 (U_kP_k^U)U_k =0.$$
This implies that
$$(U_kV_k)^2 P_k^U + \beta_1(U_k^2)P_k^U+\beta_2 U_k^2P_k^U = CU_kV_k + BU_k.$$
It follows that 
\begin{align*}
P_k^U = \frac{CU_kV_k+BU_k(\beta_1)}{U_k^2V_k^2+\beta_1U_k^2+\beta_2U_k^2}, \hspace{3mm} U_{k+1} = \frac{CV_k+B(\beta_1)}{V_k^2+\beta_1+\beta_2}.
\end{align*}
Vectorization of the above leads to the following. 
\begin{align}
U_{k+1} = [U_k]^{ij} \left[ \frac{CU_k^T+\beta_1 B}{U_kV_kV_k^T + \beta_1 U_k +\beta_2 U_k}\right]^{ij}, \hspace{3mm} \text{or} \hspace{3mm} U_{k+1} = \left[U_k\right]_{ij}  \frac{ \left[ CU_k^T+\beta_1 B \right]_{ij}}{ \left[U_kV_kV_k^T + \beta_1 U_k +\beta_2 U_k\right]_{ij}}.
\label{eq:1}
\end{align}
\newpage
On a similar note, 
\begin{align}
V_{k+1} = = \left[V_k\right]_{ij}  \frac{ \left[ U_k^TC \right]_{ij}}{ \left[U_k^TU_kV_k + \beta_3 V_k \right]_{ij}}.
\label{eq:2}
\end{align}
For L-1 Norm, say:
$$ \frac{d (|x|)}{dx} = \frac{|x|}{x} = \left\{ \begin{array}{cc} 1, & x > 0 \\ -1, & x \leq 0 \end{array} \right\}.$$
Replacing $\frac{\beta}{2} ||U||_F^2$ by $\beta_2 ||U||_1$ and $\frac{\beta_3}{2} ||V||_F^2$ by $\beta_3 ||V||_1$, we have 
\begin{align*}
\left[ U_{k+1} \right]_{ij}  = \max \left[ (\ref{eq:1}), 0 \right] \\ 
\left[ V_{k+1} \right]_{ij}  = \max \left[ (\ref{eq:2}), 0 \right].
\end{align*}

\paragraph{Backtracking:}
Let us define a direction $d_k^U$ as follows in reference to the problem in only $U$ above.
$$d_k^U = x_kP_k^U-x_k.$$
Let us define our iterates as follows.
$$x_{k+1} = x_k+\alpha d_k^U.$$ 
To find an optimal $\alpha$, given a scalar problem it then suffices to look into the case below.
$$\min_{\alpha} \left(c-uv-uv(p-1)\alpha\right)^2+(u+u(p-1)\alpha)^2+(u-B+u\alpha(p-1))^2.$$
Taking the first order conditions, it follows that
$$2u^2v^2(p-1)^2\alpha -2uv(p-1)(c-uv)+2u^2(p-1)^2\alpha+2u^2(p-1)+2u^2(p-1)^2\alpha+2u(u-B)(p-1)=0.$$
This further implies that
\begin{align*}
\alpha = \frac{v(c-uv)-2u+-B}{uv^2(p-1)+4u(p-1)}.
\end{align*}
Extending this to matrices,
$$ \alpha = \frac{\|2V(C-UV^T)-4U+2B\|_{F}}{\|UVV^T(P-ee^T)+(U+U^T)(P-ee^T) \|_F}.$$
Note that U, V, and C are all of the same dimensions. Also $e$ is a vector of ones defined appropriately.
We note that while the above is easily intuitive, the formal proof is not obvious. We do not provide the same in this version and this is given as a practical numerical enhancement. 
\section{Proofs}
\begin{lemma}
Let $U \in \mathbb{R}^{2 \times 2}$ and let $C \in \mathbb{R}^{2 \times 2}$. Let additionally, U and C have similar rows (Row 1 == Row 2). Let  $\beta_1 = 0$ and $\beta_2 = \beta_3 = 1$, for simplicity (though not obvious, these can be easily generalized). Then, $p_k^U$ is a direction for multiplicative descent mentioned above.
\end{lemma}
\begin{proof}
Let without loss of generality, 
$$ C = \pmat{c_1 & c_2 \\ c_3 & c_4}, \text{and} U = \pmat{u_1 & u_2 \\ u_3 & u_4}.$$
Noting the problem only in $U$, it can be observed that
$$P_k^U = \pmat{\frac{c_1u_1+c_2u_2}{2u_1} &  \frac{c_1u_3+c_2u_4}{2u_2} \\ \frac{c_3u_1+c_4u_2}{2u_3} & \frac{c_3u_3+c_4u_4}{2u_4}}.$$
The required portion of the objective in U can be defined as follows.
$$f(U,C) = \frac{1}{2} \left(c_1^2+c_2^2+c_3^2+c_4^2+2u_1^2+2u_2^2+2u_3^2+2u_4^2 - 2c_1u_1-2c_2u_2-2c_3u_3-2c4u_4 \right).$$
Similarly, 
\begin{align*}
f(UP_k^U,C) &= \frac{1}{2} \left( c_1^2+c_2^2+c_3^2+c_4^2 +\frac{1}{2} \left[ (c_1u_1+c_2u_2)^2 + (c_1u_3+c_2u_4)^2 + (c_3u_1+c_4u_2)^2\right] \right) \\ 
&+\frac{1}{4} \left( \left[ (c_3u_3+c_4u_4)^2\right]\right)
+\frac{1}{2}\left(-c_1(c_1u_1+c_2u_2)-c_2(c_1u_3+c_2u_4) \right) \\
&+\frac{1}{2} \left(-c_3(c_3u_1+c_4u_2)-c_4(c_3u_3+c_4u_4)\right).
\end{align*}
Noting $R_1 == R_2$ in both $C$ and $U$, it follows that $u_1 = u_3, u_2 = u_4, c_1 = c_3$, and $c_2 = c_4$. It further follows that, 
$$f(UP_k^U,C) = \left(c_1u_1+c_2u_2\right) \left( c_1u_1+c_2u_2-c_1-c_2\right).$$
It is also easy to observe that 
$$f(U,C) = u_1^2-2c_1u_1+u_2^2-2c_2u_2.$$
It is easily observed that for any $C_ij, U_ij \geq 1$, 
$$ f(UP_k^U,C) \leq f(U,C).$$ 
Our claim follows. 
\end{proof}
%\closing{To be Added:}
%\encl{To be Added:} % List your enclosed documents here, comment this out to get rid of the "encl:"
%----------------------------------------------------------------------------------------
%\end{letter}
\end{document} 
